Sensitivity Analysis for Markov Decision Process Congestion Games

We consider a non-atomic congestion game where each decision maker performs selfish optimization over states of a common MDP. The decision makers optimize for their own expected costs, and influence each other through congestion effects on the state-action costs. We analyze on the sensitivity of MDP congestion game equilibria to uncertainty and perturbations in the state-action costs by applying an implicit function type analysis. The occurrence of a stochastic Braess paradox is defined, analyzed based on sensitivity of game equilibria and demonstrated in simulation. We further analyze how the introduction of stochastic dynamics affects the magnitude of Braess paradox in comparison to deterministic dynamics.

==> nonatomicCongestionGame.tex <==
\section{Nonatomic MDP Congestion Games}\label{sec:nonatomicCongestionGame}
% \subsection{Notation}

% Define graph $G$ on the probability tensor $P$, such that the vertices of the graph are $\mc{S}$. An edge exists between $s'$ and $s$ for each $(a,s')$ where $P_{sas'} > 0$. We represent the flow on the edges by $y = \begin{pmatrix}y_{s_1a_1}, y_{s_1a_2}, \ldots y_{s_1a_m}, \ldots y_{s_na_1},\ldots y_{s_na_m}\end{pmatrix}^T$. Then $y_{s_ia_j}$ represents the portion of total population who are in state $s_i$ and chose $a_j$. Note that $y$ implicitly defines policy. 

% % The \emph{transition matrix} $\bar{P}$ transfers flow from one time step to the next. Let $P_{sa}(s') = P_{s'as}$, and $P(s') \in \reals^{|\mc{S}|\times|\mc{A}|}$ be the matrix version. Then the transition matrix is defined as
% % \[\bar{P} = \begin{pmatrix}\text{vec}(P(s_1))^T \\\text{vec}(P(s_2))^T\\ \vdots \\\text{vec}(P(s_n))^T \end{pmatrix} \]
% Let flow in time $k$ be $y^k$, the flow in time step $k+1$ is $y^{k+1} = \bar{P}y^k$. 

% \subsection{MDP Congestion Game}
Consider a MDP Congestion game where we are minimizing the infinite horizon average cost, played by a continuous population $M> 0$.  Each individual player would solve the following MDP problem: 
\begin{subequations}\label{eqn:individualCG}
\begin{align}
\underset{x_{sa}}{\min} & \sum_{sa} x_{sa}\ell_{sa}(y_{sa}) \\
\text{s.t. } & \sum_a x_{sa} =  \sum_{s', a} P_{sas'}x_{s'a}, \\
& \sum_{a}x_{sa} = 1, \\
& x_{sa} \geq 0, \quad \forall t \in [T], s \in \mc{S}, a \in \mc{A}    
\end{align}
\end{subequations}
Where $x$ is the policy undertaken by an individual player, $y_{sa}$ is the total mass density at the current state action pair. 

The equilibrium mass distribution of such a game is equivalently the equilibrium solution to the following potential game. 
\begin{subequations}
\begin{align}
\underset{y}{\min} & \quad \sum\limits_{s\in\mathcal{S}} \sum\limits_{a\in\mathcal{A}} \int_0^{y_{sa}}\ell_{sa}(x)dx \\
\mbox{s.t.} & \quad Ey = 0\\ 
& \quad \ones^Ty = M\\
& \quad y \geq 0 \\
\end{align}
\label{eqn:mdpgame}
\end{subequations}
Where $\ell_{sa}: \reals_+ \rightarrow \reals$ defines the congestion effects on edge $k = (s,a)$ as a function of its current mass density. Assuming that more mass on any given state-action edge will cause congestion and increase the cost of taking the edge, we can make the following assumption. 
\begin{assumption}
\label{ass:increasing}
$\ell_{tsa}(u): \reals_+ \rightarrow \reals$ is strictly increasing for each $t \in [T]$, $a \in \mc{A}$, $s \in \mc{S}$. 
\end{assumption}
% In an MDP congestion game,we are looking for a time invariant flow distribution, ie $\bar{P}y = y$, such that no player can achieve a better incurred cost. Constraints on the flow feasibility are that the total mass is conserved, $\ones^Ty = M$, strictly positive flows, $y \geq 0$. Define $F = I_n \otimes \ones_m^T - \bar{P}$, note that $F$ is also the incidence matrix of a stochastic hypergraph.  
Let $\ell = \text{vec}(\ell_{sa})$, at optimal solution $y^\star$, $\nu^\star \in \reals^{|S|}$, $\lambda^\star \in \reals$, $\mu^\star \in \reals^{|\mc{S}|\times |\mc{A}|}$.  
\begin{subequations}
\begin{align}
\ell(y^\star) - E^T\nu^\star - \lambda^\star\ones - \mu^\star & = 0 \\
Ey^\star & = 0 \\
\ones^Ty^\star - M & = 0 \\
(\mu^\star)^T y^\star & = 0 \\
\mu^\star & \geq 0 
\end{align}
\end{subequations}
Each dual variable has a unique game interpretations. $\nu$ can be interpreted as \emph{state potentials} defined for each vertex, $E^T\nu$ can be interpreted as the expected change in potential in taking action $a$ to reach state $s$.
\[(E^T\nu)_{(s,a)} = \nu_s - \underset{s'}{\sum} P_{s' a}(s) \nu_{s'}\]
Then from the first KKT condition, we can directly solve for state potentials: 
\[\nu^\star_s = \underset{a}{\min} \,\ell_{sa}(y^\star_{sa}) + \underset{s'}{\sum} P_{s' a}(s) \nu^\star_{s'} + \lambda^\star\]
Where $\ell_{sa}(y^\star_{sa}) $ is the immediate cost of taking an edge, and $ \underset{s'}{\sum} P_{s' a}(s) \nu^\star_{s'}$ is the expected potential by taking action $a$. 

Suppose we compute the density weighted overall sum, $ y^TF^T\nu^\star = 0$ 
\[y^T \ell(y^\star) = y^T\ones \lambda = M \lambda\]
Then $\lambda$ is the \emph{average cost}, the necessary cost incurred on each edge. 

\begin{definition}[Wardrop Equilibrium]
A population mass distribution $y^\star$ is a stationary infinite horizon Wardrop equilibrium with corresponding state potentials $\nu^\star(y^\star)$ defined by the KKT conditions, if for all other feasible $y$, 
\[\nu^\star(y^\star) \leq \nu(y) \quad \forall s \in \mc{S}\]
\end{definition}
This can be derived from the KKT conditions. 

We can see that the set of Wardrop equilibrium points coincides with the optimal solution to the optimization problem. An alternative but equivalent characterization is a Variational Inequality (VI). Network flow problems were first introduced as Variational Inequalities by DAFERMOS. Here we specify the definition for an MDP Congestion game. 

\begin{definition}[Variational Inequality: Wardrop Equilibrium]
Let the set of feasible population be defined as the following:
\[K = \{y | Ey = 0,\,\,\ones^Ty - M = 0,\,\, y \geq 0 \} \]
Then a stationary wardrop equilibrium is defined as $y^\star \in K$ where
\[\ell(y^\star)^T(y - y^\star) \geq 0 \quad \forall y \in K\]
\end{definition}
\begin{proof}{$\ell(y^\star)^T(y - y^\star) $ is equivalent to the directional derivative of $f(y) = \int^{y^\star}_0\ell(u)\partial u$, written as $f'(y^\star; d)$ where $d = y - y^\star$. Since the directional derivative is continuous for all $y \in K$, $y^\star$ achieves minimum $f(y)$ on the convex set K. }
\end{proof}
